Stack Semantics of Type Theory

We give a model of dependent type theory with one univalent universe and propositional truncation interpreting a type as a stack, generalising the groupoid model of type theory. As an application, we show that countable choice cannot be proved in dependent type theory with one univalent universe and propositional truncation.

==> aliases <==
\newcommand{\UU}{\Univ}
\newcommand{\NN}{\Nat}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\rats}{\mathbb{Q}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\norm}[1]{\Trunc{#1}}


==> unicode-math-table <==
\DeclareUnicodeCharacter{000AC}{\neg              }
\DeclareUnicodeCharacter{000B7}{\cdot             }
\DeclareUnicodeCharacter{000D7}{\times            }
\DeclareUnicodeCharacter{00391}{A                 }
\DeclareUnicodeCharacter{00392}{B                 }
\DeclareUnicodeCharacter{00393}{\Gamma            }
\DeclareUnicodeCharacter{00394}{\Delta            }
\DeclareUnicodeCharacter{00395}{E                 }
\DeclareUnicodeCharacter{00396}{Z                 }
\DeclareUnicodeCharacter{00397}{H                 }
\DeclareUnicodeCharacter{00398}{\Theta            }
\DeclareUnicodeCharacter{00399}{I                 }
\DeclareUnicodeCharacter{0039A}{K                 }
\DeclareUnicodeCharacter{0039B}{\Lambda           }
\DeclareUnicodeCharacter{0039C}{M                 }
\DeclareUnicodeCharacter{0039D}{N                 }
\DeclareUnicodeCharacter{0039E}{\Xi               }
\DeclareUnicodeCharacter{0039F}{O                 }
\DeclareUnicodeCharacter{003A0}{\Pi               }
\DeclareUnicodeCharacter{003A1}{P                 }
\DeclareUnicodeCharacter{003A3}{\Sigma            }
\DeclareUnicodeCharacter{003A4}{T                 }
\DeclareUnicodeCharacter{003A5}{\Upsilon          }
\DeclareUnicodeCharacter{003A6}{\Phi              }
\DeclareUnicodeCharacter{003A7}{X                 }
\DeclareUnicodeCharacter{003A8}{\Psi              }
\DeclareUnicodeCharacter{003A9}{\Omega            }
\DeclareUnicodeCharacter{003B1}{\alpha            }
\DeclareUnicodeCharacter{003B2}{\beta             }
\DeclareUnicodeCharacter{003B3}{\gamma            }
\DeclareUnicodeCharacter{003B4}{\delta            }
\DeclareUnicodeCharacter{003B5}{\epsilon          }
\DeclareUnicodeCharacter{003B6}{\zeta             }
\DeclareUnicodeCharacter{003B7}{\eta              }
\DeclareUnicodeCharacter{003B8}{\theta            }
\DeclareUnicodeCharacter{003B9}{\iota             }
\DeclareUnicodeCharacter{003BA}{\kappa            }
\DeclareUnicodeCharacter{003BB}{\lambda           }
\DeclareUnicodeCharacter{003BC}{\mu               }
\DeclareUnicodeCharacter{003BD}{\nu               }
\DeclareUnicodeCharacter{003BE}{\xi               }
\DeclareUnicodeCharacter{003BF}{\omicron          }
\DeclareUnicodeCharacter{003C0}{\pi               }
\DeclareUnicodeCharacter{003C1}{\rho              }
\DeclareUnicodeCharacter{003C3}{\sigma            }
\DeclareUnicodeCharacter{003C4}{\tau              }
\DeclareUnicodeCharacter{003C5}{\upsilon          }
\DeclareUnicodeCharacter{003C6}{\varphi           }
\DeclareUnicodeCharacter{003C7}{\chi              }
\DeclareUnicodeCharacter{003C8}{\psi              }
\DeclareUnicodeCharacter{003C9}{\omega            }
\DeclareUnicodeCharacter{02016}{\Vert             }
\DeclareUnicodeCharacter{02026}{\ldots            }
\DeclareUnicodeCharacter{02102}{\mathbb{C}        }
\DeclareUnicodeCharacter{0210D}{\mathbb{H}        }
\DeclareUnicodeCharacter{02115}{\mathbb{N}        }
\DeclareUnicodeCharacter{02119}{\mathbb{P}        }
\DeclareUnicodeCharacter{0211A}{\mathbb{Q}        }
\DeclareUnicodeCharacter{0211D}{\mathbb{R}        }
\DeclareUnicodeCharacter{02124}{\mathbb{Z}        }
\DeclareUnicodeCharacter{02190}{\leftarrow        }
\DeclareUnicodeCharacter{02191}{\uparrow          }
\DeclareUnicodeCharacter{02192}{\rightarrow       }
\DeclareUnicodeCharacter{02193}{\downarrow        }
\DeclareUnicodeCharacter{02194}{\leftrightarrow   }
\DeclareUnicodeCharacter{02195}{\updownarrow      }
\DeclareUnicodeCharacter{021A4}{\mapsfrom         }
\DeclareUnicodeCharacter{021A5}{\mapsup           }
\DeclareUnicodeCharacter{021A6}{\mapsto           }
\DeclareUnicodeCharacter{021A7}{\mapsdown         }
\DeclareUnicodeCharacter{021D0}{\Leftarrow        }
\DeclareUnicodeCharacter{021D1}{\Uparrow          }
\DeclareUnicodeCharacter{021D2}{\Rightarrow       }
\DeclareUnicodeCharacter{021D3}{\Downarrow        }
\DeclareUnicodeCharacter{021D4}{\Leftrightarrow   }
\DeclareUnicodeCharacter{021D5}{\Updownarrow      }
\DeclareUnicodeCharacter{02200}{\forall           }
\DeclareUnicodeCharacter{02203}{\exists           }
\DeclareUnicodeCharacter{02205}{\emptyset         }
\DeclareUnicodeCharacter{02208}{\in               }
\DeclareUnicodeCharacter{02216}{\setminus         }
\DeclareUnicodeCharacter{02217}{\ast              }
\DeclareUnicodeCharacter{02218}{\circ             }
\DeclareUnicodeCharacter{02219}{\bullet           }
\DeclareUnicodeCharacter{02227}{\wedge            }
\DeclareUnicodeCharacter{02228}{\vee              }
\DeclareUnicodeCharacter{02229}{\cap              }
\DeclareUnicodeCharacter{0222A}{\cup              }
\DeclareUnicodeCharacter{0222B}{\int              }
\DeclareUnicodeCharacter{02241}{\nsim             }
\DeclareUnicodeCharacter{02242}{\eqsim            }
\DeclareUnicodeCharacter{02243}{\simeq            }
\DeclareUnicodeCharacter{02244}{\nsime            }
\DeclareUnicodeCharacter{02245}{\cong             }
\DeclareUnicodeCharacter{02247}{\ncong            }
\DeclareUnicodeCharacter{02248}{\approx           }
\DeclareUnicodeCharacter{02249}{\napprox          }
\DeclareUnicodeCharacter{0224A}{\approxeq         }
\DeclareUnicodeCharacter{02254}{\coloneq          }
\DeclareUnicodeCharacter{02255}{\eqcolon          }
\DeclareUnicodeCharacter{02260}{\ne               }
\DeclareUnicodeCharacter{02261}{\equiv            }
\DeclareUnicodeCharacter{02262}{\nequiv           }
\DeclareUnicodeCharacter{02264}{\leq              }
\DeclareUnicodeCharacter{02265}{\geq              }
\DeclareUnicodeCharacter{02282}{\subset           }
\DeclareUnicodeCharacter{02283}{\supset           }
\DeclareUnicodeCharacter{02286}{\subseteq         }
\DeclareUnicodeCharacter{02287}{\supseteq         }
\DeclareUnicodeCharacter{0228A}{\subsetneq        }
\DeclareUnicodeCharacter{0228B}{\supsetneq        }
\DeclareUnicodeCharacter{022A2}{\vdash            }
\DeclareUnicodeCharacter{022A3}{\dashv            }
\DeclareUnicodeCharacter{022A4}{\top              }
\DeclareUnicodeCharacter{022A5}{\bot              }
\DeclareUnicodeCharacter{022C0}{\bigwedge         }
\DeclareUnicodeCharacter{022C1}{\bigvee           }
\DeclareUnicodeCharacter{022C2}{\bigcap           }
\DeclareUnicodeCharacter{022C3}{\bigcup           }
\DeclareUnicodeCharacter{022C6}{\star             }
\DeclareUnicodeCharacter{027E8}{\langle           }
\DeclareUnicodeCharacter{027E9}{\rangle           }
\DeclareUnicodeCharacter{027EA}{\lAngle           }
\DeclareUnicodeCharacter{027EB}{\rAngle           }
\DeclareUnicodeCharacter{02972}{\similarrightarrow}
\DeclareUnicodeCharacter{02A7D}{\leqslant         }
\DeclareUnicodeCharacter{02A7E}{\geqslant         }
\DeclareUnicodeCharacter{1D538}{\mathbb{A}        }
\DeclareUnicodeCharacter{1D539}{\mathbb{B}        }
\DeclareUnicodeCharacter{1D53B}{\mathbb{D}        }
\DeclareUnicodeCharacter{1D53C}{\mathbb{E}        }
\DeclareUnicodeCharacter{1D53D}{\mathbb{F}        }
\DeclareUnicodeCharacter{1D53E}{\mathbb{G}        }
\DeclareUnicodeCharacter{1D540}{\mathbb{I}        }
\DeclareUnicodeCharacter{1D541}{\mathbb{J}        }
\DeclareUnicodeCharacter{1D542}{\mathbb{K}        }
\DeclareUnicodeCharacter{1D543}{\mathbb{L}        }
\DeclareUnicodeCharacter{1D544}{\mathbb{M}        }
\DeclareUnicodeCharacter{1D546}{\mathbb{O}        }
\DeclareUnicodeCharacter{1D54A}{\mathbb{S}        }
\DeclareUnicodeCharacter{1D54B}{\mathbb{T}        }
\DeclareUnicodeCharacter{1D54C}{\mathbb{U}        }
\DeclareUnicodeCharacter{1D54D}{\mathbb{V}        }
\DeclareUnicodeCharacter{1D54E}{\mathbb{W}        }
\DeclareUnicodeCharacter{1D54F}{\mathbb{X}        }
\DeclareUnicodeCharacter{1D550}{\mathbb{Y}        }
\DeclareUnicodeCharacter{1D552}{\mathbb{a}        }
\DeclareUnicodeCharacter{1D553}{\mathbb{b}        }
\DeclareUnicodeCharacter{1D554}{\mathbb{c}        }
\DeclareUnicodeCharacter{1D555}{\mathbb{d}        }
\DeclareUnicodeCharacter{1D556}{\mathbb{e}        }
\DeclareUnicodeCharacter{1D557}{\mathbb{f}        }
\DeclareUnicodeCharacter{1D558}{\mathbb{g}        }
\DeclareUnicodeCharacter{1D559}{\mathbb{h}        }
\DeclareUnicodeCharacter{1D55A}{\mathbb{i}        }
\DeclareUnicodeCharacter{1D55B}{\mathbb{j}        }
\DeclareUnicodeCharacter{1D55C}{\mathbb{k}        }
\DeclareUnicodeCharacter{1D55D}{\mathbb{l}        }
\DeclareUnicodeCharacter{1D55E}{\mathbb{m}        }
\DeclareUnicodeCharacter{1D55F}{\mathbb{n}        }
\DeclareUnicodeCharacter{1D560}{\mathbb{o}        }
\DeclareUnicodeCharacter{1D561}{\mathbb{p}        }
\DeclareUnicodeCharacter{1D562}{\mathbb{q}        }
\DeclareUnicodeCharacter{1D563}{\mathbb{r}        }
\DeclareUnicodeCharacter{1D564}{\mathbb{s}        }
\DeclareUnicodeCharacter{1D565}{\mathbb{t}        }
\DeclareUnicodeCharacter{1D566}{\mathbb{u}        }
\DeclareUnicodeCharacter{1D567}{\mathbb{v}        }
\DeclareUnicodeCharacter{1D568}{\mathbb{w}        }
\DeclareUnicodeCharacter{1D569}{\mathbb{x}        }
\DeclareUnicodeCharacter{1D56A}{\mathbb{y}        }
\DeclareUnicodeCharacter{1D56B}{\mathbb{z}        }

